Automated Application Offloading through Ant-inspired Decision-Making

-The explosive trend of smartphone usage as the most effective and convenient communication tools of human life in recent years make developers build ever more complex smartphone applications. Gaming, navigation, video editing, augmented reality, and speech recognition applications require considerable computational power and energy. Although smart- phones have a wide range of capabilities - GPS, WiFi, cameras - their inherent limitations - frequent disconnections, mobility - and significant constraints - size, lower weights, longer battery life - make difficult to exploiting their full potential to run complex applications. Several research works have proposed solutions in application offloading domain, but few ones concerning the highly changing properties of the environment. To address these issues, we realize an automated application offloading middleware, ACOMMA, with dynamic and re-adaptable decision-making engine. The decision engine of ACOMMA is based on an ant- inspired algorithm.

==> Makefile <==
#
# latex2e Makefile
#

#
# Variables
#

#
# Environment variables
#

CD    = cd
CHMOD = chmod
FIND  = find
LN    = ln
MV    = mv
RM    = rm

#
# Prog variables
#

LATEX       = latex
BIBTEX      = bibtex
XDVI        = xdvi
DVI2PS      = dvips
DVI2PDF     = dvipdf
TEX2HTML    = latex2html -no_navigation -split 0 -address "frederic.le-mouel@insa-lyon.fr (C)INSA Lyon 2011"

.SUFFIXES: .tex .bib .aux .bbl .dvi .eps .fig .ps .pdf .html

#
# LaTeX file variables
#

TXT_FILE1 = NOTERE-AntInspiredMobileOffloading

LATEX_FILE1  = $(TXT_FILE1).tex
BIBTEX_FILE1 = $(TXT_FILE1).bib

AUX_FILE1 = $(TXT_FILE1).aux
BIB_FILE1 = $(TXT_FILE1).bbl
BLG_FILE1 = $(TXT_FILE1).blg
BRF_FILE1 = $(TXT_FILE1).brf
LOG_FILE1 = $(TXT_FILE1).log
LOT_FILE1 = $(TXT_FILE1).lot
LOF_FILE1 = $(TXT_FILE1).lof
OUT_FILE1 = $(TXT_FILE1).out
DVI_FILE1 = $(TXT_FILE1).dvi

#
# Figures variables
#

FIG_DIR = ./figures

#
# Outputs files variables
#

PS_FILE1  = $(TXT_FILE1).ps

PDF_FILE1 = $(TXT_FILE1).pdf

HTML_FILE1 = $(TXT_FILE1).html

#
# Make without dependencies : let's make tex
#

make_without_dependencies: tex

#
# Let's make all
#

all: tex ps pdf html view

#
# Let's make figures
#

fig:
	( $(CD) $(FIG_DIR); $(MAKE) $(MFLAGS) fig )

#
# Let's make LaTeX file
#

#tex: fig aux bib dvi
tex: aux bib dvi

.tex.aux:
	$(LATEX) $<
	$(CHMOD) g+r $(<:.tex=.log)
	$(CHMOD) g+r $@
	$(RM) $(<:%tex=%dvi)

aux: $(AUX_FILE1)

.tex.dvi: 
	$(LATEX) $<
	$(CHMOD) g+r $(<:.tex=.log)
	$(CHMOD) g+r $(<:.tex=.aux)
	$(CHMOD) g+r $@

dvi: bib $(DVI_FILE1)

#
# Bibliography file
#

%.bbl : %.bib %.tex
	$(BIBTEX) $(<:.bib=)
	$(CHMOD) g+r $(<:.bib=.blg)
	$(CHMOD) g+r $@
	$(LATEX) $(<:%bib=%tex)
	$(CHMOD) g+r $(<:.tex=.log)
	$(CHMOD) g+r $(<:.tex=.aux)
	$(RM) $(<:%bib=%dvi)

bib: aux $(BIB_FILE1)

#
# Let's see
#

view: tex
	$(XDVI) $(DVI_FILE1) &

#
# Let's make outputs
#

#
# Postscript
#

.dvi.ps:
	$(DVI2PS) $< -o $@
	$(CHMOD) g+r $@

ps: tex $(PS_FILE1)

#
# Pdf
#

.dvi.pdf:
	$(DVI2PDF) $< $@
	$(CHMOD) g+r $@

pdf: tex $(PDF_FILE1)

#
# HTML
#

.tex.html:
	$(TEX2HTML) $<
	$(FIND) $(<:.tex=) -type d -exec $(CHMOD) g+rx {} \; -ls
	$(FIND) $(<:.tex=) -type f -exec $(CHMOD) g+r {} \; -ls
	$(LN) -s -f $(<:.tex=)/$@ $@

html: tex $(HTML_FILE1)

#
# Clean of the directory
#

#clean: clean_fig clean_tex clean_bib clean_ps clean_pdf clean_html
clean: clean_tex clean_bib clean_ps clean_pdf clean_html

clean_fig:
	( $(CD) $(FIG_DIR) ; $(MAKE) $(MFLAGS) clean_fig )

clean_tex:
	$(RM) -f $(AUX_FILE1) $(LOG_FILE1) $(LOT_FILE1) $(LOF_FILE1) $(DVI_FILE1) $(OUT_FILE1) $(BRF_FILE1) $(TXT_FILE1).idx $(TXT_FILE1).toc

clean_bib:
	$(RM) -f $(BIB_FILE1) $(BLG_FILE1)

clean_ps:
	$(RM) -f $(PS_FILE1)

clean_pdf:
	$(RM) -f $(PDF_FILE1)

clean_html:
	$(RM) -rf $(TXT_FILE1) $(HTML_FILE1)


